Clarification on the Mapping of Reversible Circuits to the NCV-v1 Library

In previous work and motivated by a theoretical discussion on physical realizations, a new quantum gate library (the NCV-v1 library) for electronic design automation of quantum circuits has been proposed. Here, qudits instead of qubits are assumed, i.e. a basic building block which does not rely on a two level quantum system but a (multiple-valued) d-level quantum system is assumed. However, the descriptions on the foundation of this new library remained brief. This technical report provides an extended description of the applied ideas and concepts.

==> makeloopPDF <==
#!/usr/bin/perl

# call make but just display the lines printing an error
sub make {
    open MAKE, "make pdf |";
    while (<MAKE>)
    {
        print $_ if ( /(^[^:]+:\d+: .*$)|^l\./ );
    }
    close MAKE;
}

if ( !@ARGV )
{
    print "  usage: $0 file\n";
    print "  where file is the top tex file without file extension tex\n";
    print "  starts okular for file and calls make command every time a tex file changes\n";
    exit;
}

my $filebase = shift;
my $viewer   = "okular";

make;

my $pid = fork();
if ( !$pid )
{
    exec( "$viewer $filebase.pdf > /dev/null 2>&1" );
    die;
}
else
{
    $SIG{CHLD} = 'IGNORE';
    while ( 1 ) {
        @ft = `bash -c "if [ -N $filebase.tex ]; then echo 1; fi"`;
        make if @ft;
        system( "sleep 1" );

        $running = kill 0, $pid;
        last if !$running;
    }
}

